OnePerc: A Randomness-aware Compiler for Photonic Quantum Computing

The photonic platform holds great promise for quantum computing. Nevertheless, the intrinsic probabilistic characteristics of its native fusion operations introduces substantial randomness into the computing process, posing significant challenges to achieving scalability and efficiency in program execution. In this paper, we introduce a randomness-aware compilation framework designed to concurrently achieve scalability and efficiency. Our approach leverages an innovative combination of offline and online optimization passes, with a novel intermediate representation serving as a crucial bridge between them. Through a comprehensive evaluation, we demonstrate that this framework significantly outperforms the most efficient baseline compiler in a scalable manner, opening up new possibilities for realizing scalable photonic quantum computing.

==> commands.tex <==
\usepackage{float}
\usepackage{stfloats}
\usepackage{titlesec}
\DeclareUnicodeCharacter{2009}{\,} 
\titlespacing*{\section}
{0pt}{\parsep}{\parsep}
\titlespacing*{\subsection}
{0pt}{\parsep}{\parsep}
\usepackage{xcolor}

\newcommand\bra[1]{\left\langle#1\right|}
\newcommand\ket[1]{\left|#1\right\rangle}
\newcommand\norm[1]{\left|#1\right|}




\usepackage{amsmath,mathtools, amssymb, amsthm}
\newtheorem{definition}{Definition}[section]
\newtheorem{theorem}{Theorem}[section]
% \newtheorem{proof}{Proof}[section]
\newtheorem{proposition}{Proposition}[section]
\newcommand\todo[1]{\textcolor{red}{#1}}
\newcommand\Hezi[1]{\textcolor{purple}{#1}}
\newcommand\yuke[1]{\textcolor{blue}{\textbf{[Yuke: #1]}}}
\newcommand\hz[1]{\textcolor{purple}{\textbf{[HZ: #1]}}}
\newcommand{\GL}[1]{\textcolor{red} {G.L.: #1}}
\newcommand*{\HS}[1]{\textcolor{blue}{[HS: #1]}}
\newcommand\fix[1]{\textcolor{blue}{#1}}
\newcommand\fixmore[1]{\textcolor{red!70!black}{#1}}

\usepackage[normalem]{ulem}
\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
\usepackage{xcolor}
\usepackage{color}
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}
\definecolor{textblue}{rgb}{.2,.2,.7}
\definecolor{textred}{rgb}{0.54,0,0}
\definecolor{textgreen}{rgb}{0,0.43,0}
\definecolor{codered}{rgb}{201,72,12}
\usepackage[T1]{fontenc}
\usepackage[scaled=0.85]{beramono} 
\usepackage{listings}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{url}
% \usepackage{subfig}
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\usepackage{multirow}
\usepackage{tikz}
\usepackage{xcolor}
\usepackage{ctable} % for \specialrule command

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[circle,fill=.,inner sep=0.8pt] (char) {\textcolor{white}{#1}};}}

\newcommand{\frameworkname}{our framework}
\newcommand{\frameworkName}{our framework}


\newcommand{\md}[1]{\textcolor{red}{#1}}

